Generalized Representative Structures for Atomistic Systems

A new method is presented to generate atomic structures that reproduce the essential characteristics of arbitrary material systems, phases, or ensembles. Previous methods allow one to reproduce the essential characteristics (e.g. chemical disorder) of a large random alloy within a small crystal structure. The ability to generate small representations of random alloys, with the restriction to crystal systems, results from using the fixed-lattice cluster correlations to describe structural characteristics. A more general description of the structural characteristics of atomic systems is obtained using complete sets of atomic environment descriptors. These are used within for generating representative atomic structures without restriction to fixed lattices. A general data-driven approach is provided utilizing the atomic cluster expansion(ACE) basis. The N-body ACE descriptors are a complete set of atomic environment descriptors that span both chemical and spatial degrees of freedom and are used within for describing atomic structures. The generalized representative structure(GRS) method presented within generates small atomic structures that reproduce ACE descriptor distributions corresponding to arbitrary structural and chemical complexity. It is shown that systematically improvable representations of crystalline systems on fixed parent lattices, amorphous materials, liquids, and ensembles of atomic structures may be produced efficiently through optimization algorithms. We highlight reduced representations of atomistic machine-learning training datasets that contain similar amounts of information and small 40-72 atom representations of liquid phases. The ability to use GRS methodology as a driver for informed novel structure generation is also demonstrated. The advantages over other data-driven methods and state-of-the-art methods restricted to high-symmetry systems are highlighted.

==> methods_jmg.tex <==
\subsection{Fundamental methodology for GRS}
%To preface the methodology and definitions for GRS, the methods and definitions of the SQS are summarized. 
%Likewise GRS are defined as structures that minimize Eq. \eqref{eq:inter_structure}. 
%A GRS is defined as the structure that minimizes the loss function in Eq. \eqref{eq:inter_structure}.

Atomic descriptors, Eq. \ref{eq:ace_set}, can be used to represent atomic structures, and provide a convenient means to quantify similarity between structures. This was used to define the GRS loss function in the previous section. 
A structure that reproduces some targeted distribution of atomic descriptors in practice may be obtained by minimizing the GRS loss function over the positions in the structure $\boldsymbol{R}_s$ and the chemical occupations of atomic sites $\boldsymbol{\sigma}_s$.
\begin{equation}
    \min_{(\boldsymbol{R}_s,\boldsymbol{\sigma}_s)} \big[Q_{GRS}\big]
    \label{eq:grs_def}
\end{equation}
In Eq. \eqref{eq:grs_def}, a GRS is defined by minimizing the GRS loss Eq. \eqref{eq:inter_structure}. 
The GRS loss functions may be minimized provided that informed choices are made for the optimization algorithms and the initial structures.
As with SQS, the optimization algorithms and initial structures are chosen for GRS based on the target distribution and the degrees of freedom for the descriptors.
%In practice, different minimization algorithms may be used to find the best representative structure based on the target distribution. These different optimization algorithms will be highlighted in a later section along with informed choices for initial structures. 
Sets of fixed-lattice structures have been generated that have certain descriptor distributions.\cite{sorkin2020generalized} 
This is best extended to atomic systems that aren't on a fixed lattice by generating a set of GRS. 
A GRS set (GRSS) is defined by a set of structures that minimize both the inter-structure (Eq. \eqref{eq:inter_structure} and intra-structure (Eq. \eqref{eq:intra_structure}) loss.
\begin{equation}
    \min_{(R_{s_1}\sigma_{s_1}),(R_{s_2}\sigma_{s_2}), \cdots (R_{s_{N_s}}\sigma_{s_{N_s}})}\big[w_1 Q_{GRS} + w_2 Q_{GRS}^{intra} \big]
    \label{eq:grs_set_def}
\end{equation}
In Eq. \eqref{eq:grs_set_def}, a set of structures that both collectively and locally reproduce a target distribution is defined. 
Here, minimization is performed over the positions and chemical occupations of atomic sites in a collection of $N_s$ atomic structures. 
Optimization algorithms and initial structures are also chosen based on the target distribution in Eq. \eqref{eq:grs_set_def}.
%One key distinction, that will be discussed in more detail later, is that 



%%The target distribution may be that of a completely random alloy to recover traditional SQS structures, but it may also be the descriptor distribution in a liquid for example. 



%Depending on the target distribution, a candidate structure is pushed towards the target distribution of descriptors by (1) varying the discrete chemical occupancy of the atomic sites, (2) varying the continuous atomic positions and cell vectors, or (3) both. 
%To find a GRS, the domain to be sampled is by definition infinite. In order to tractably obtain GRS in practice, some domain expertise is needed regarding the proposal of starting structures, optimization algorithms, and efficient methods for evaluating ACE descriptors and the associated GRS loss functions are necessary. Where we demonstrate this method, these considerations will be highlighted.


\subsection{Dynamic Minimization of GRS Loss}

To tractably minimize the GRS loss functions, algorithms will need to take advantage of the continuous differentiable ACE descriptors to move atomic positions. 
Methods for sampling chemical degrees of freedom in atomic systems are typically well-established stochastic approaches, but this is not efficient for the continuous domain of atomic positions that need to be sampled in GRS methods. 
Relying entirely on stochastic methods for both degrees of freedom would be too slow. 
Thus, we provide practical implementations of the GRS methods that enable computationally efficient optimization of the GRS loss functions through conjugate gradient and steepest descent methods.
This is done simply by treating the GRS loss functions as interatomic potentials for use in well-established molecular dynamics code bases.\cite{thompson2022lammps}

The key advance enabling optimization of GRS loss functions with dynamic atomic positions is the new ACE capabilities in the machine-learned interatomic potential (ML-IAP) interface in LAMMPS.
This interface uses efficient kernels to evaluate ACE descriptors,\cite{lysogorskiy_performant_2021} while allowing for convenient definitions of atomic interaction models as Python functions. 
This enables users to rapidly test and evaluate candidate ACE models with significant flexibility in model form.
This flexiblity is used to define GRS loss functions as effective interaction models, again emphasizing the lack of a need for true energy models for GRS.
%Atomic positions may be evolved according to GRS effective potentials in LAMMPS. 
%Minimizing the GRS loss is as simple as minimizing the effective potential with respect to atomic positions for the functions. 
%The effective potentials are defined to enable efficient minimization of GRS loss functions with respect to atomic positions, but they may still be used as loss functions for minimizing the GRS loss with respect to chemical occupations of atomic sites. 
%mall adaptations of the GRS loss functions are made to use them as effective potentials. 

The GRS effective potential in LAMMPS is defined as a function of all atomic positions, $\boldsymbol{R}_s$ as well as the chemical occupations of atomic sites, $\boldsymbol{\sigma}_s$, in structure $s$.
\begin{equation}
    V^{eff}(\boldsymbol{R}_s,\boldsymbol{\sigma} _s)=V_{core}(\boldsymbol{R}_s,\boldsymbol{\sigma}_s)  + Q_{GRS}(\boldsymbol{R}_s,\boldsymbol{\sigma}_s )
    \label{eq:single_eff}
\end{equation}
The effective potential is defined in terms of the inter-structure loss, $Q_{GRS}$, with an added interaction that eliminates atomic overlap, $V_{core}({\boldsymbol{R}_s},\boldsymbol{\sigma}_s )$. 
This is a soft-core repulsion potential, and is added such that it does not contribute significantly to the GRS loss function at physically realistic interatomic distances.
%A GRS may be found by minimizing the effective potential, Eq. \eqref{eq:single_eff}, in LAMMPS. 
The effective potential in Eq. \eqref{eq:single_eff} defined through the LAMMPS Python interface is immediately compatible with LAMMPS optimization methods and all additional simulation algorithms. 

%%%%%%%%
%Depending on the target distribution specified for $Q_{GRS}$, an optimization algorithm may be specified. Target distributions corresponding to fixed atomic positions are assigned stochastic algorithms, similar to SQS.
%If one were to only use global optimization methods, it may take a long time to find a minimum on the GRS loss surface when the targeted ACE descriptor distribution corresponds to more exotic atomic structures. 
%This is due to the infinite spatial degrees of freedom for atomic sites.
%Thus, global optimization algorithms are combined with computationally efficient local optimization algorithms in LAMMPS.
%Combining these optimization methods allows one to find reasonable representative structures for widely varied target distributions. 
%The global optimization method used to obtain GRS in practice are typically simulated annealing with Markov chains, genetic algorithms, or parallel sampling approaches.
%After (or during) a global optimization method such as annealing, states sampled in the global searches are pushed towards local minima with conjugate gradient (CG). 

%%%%%%%%

An effective potential may also be defined that facilitates the generation of multiple structures that independently and/or collectively represent a target distribution of ACE descriptors. 
This variation of the GRS loss functions is typically what is used in practice to generate GRSS.
The effective potential for GRSS is made by combining both inter and intra-structure loss functions while penalizing atomic overlap.
\begin{equation}
    \begin{split}
    &V^{eff}({\{ \boldsymbol{R}}\}_S,\{\boldsymbol{\sigma}\}_S )=V_{core}({\boldsymbol{R}},\boldsymbol{\sigma})  + w_{1}Q_{GRS}({\boldsymbol{R}_s},\boldsymbol{\sigma}_s ) \\
    & + w_{2}Q_{GRS}^{intra}({\{ \boldsymbol{R}}\}_S,\{\boldsymbol{\sigma}\}_S )
    \end{split}
    \label{eq:multi_eff}
\end{equation}
%In Eq. \eqref{eq:multi_eff}, the multi-structure effective potential is defined in terms of inter-structure as well as intra-structure loss contributions. 
This allows one to generate atomic structures that both individually and collectively reproduce a target distribution of fingerprints. 
The weights, $w_1$ and $w_2$, allow for an adjustable inter versus intra-structure similarity.
Methods to minimize the GRSS effective potential are offered in place of expensive global optimization algorithms that find a single GRS structure.
A set of representative structures may be found by starting with one GRS, adding new candidate structures to the set $S$, and evolving atomic positions such that they minimize the effective potential Eq. \eqref{eq:multi_eff}.
%Through the new ML-IAP interface in LAMMPS, the optimization of the individual candidate structures added to the set may be performed using LAMMPS optimization algorithms.


Local minima may easily be found on the GRS or GRSS loss surfaces, Eqs. \eqref{eq:single_eff} and \eqref{eq:multi_eff}, by optimizing atomic positions according to conjugate gradient (CG), steepest descent algorithms, and other optimization algorithms used for molecular dynamics.
In practice, this is combined with stochastic methods or other methods capable of finding global minima. 
The local optimization of the GRS or GRSS loss functions is wrapped by a method like (simulated) annealing, genetic algorithms, or parallel sampling. 
These are combined in different ways depending on the system, as encoded by the targeted ACE descriptor distribution. 
Details on which methods are used or combined are provided for some archetypal cases.



A case that exercises the novel capability of GRS to  represent amorphous or liquid structures is considered. 
This is done to show the most general (and difficult) approach for generating GRS requiring both global and local optimization. 
In Fig. \ref{fig:min_method}, a liquid Ta system at 4000 K is set as the target.
In this figure, a reasonable 40-atom candidate structure (grey circle) may be evolved on the GRS loss surface (illustrated as a blue line). This atomic system is firstly evolved according to a global optimization method like annealing (blue circles on the loss surface) followed by a local minimization method like CG (orange circles). 
Combining local and global optimization procedures like this allows one to find good local minima, and often global minima. In either case, the result is accurate representations of the large-scale liquid Ta target (purple star).

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{GRS_min.001.jpeg}
    \caption{Illustration that highlights the optimization of the GRS loss function for a single atomic structure. An initial structure is annealed on the loss surface are by varying atomic positions and chemical occupations (encoded in the fingerprints on the x-axis). After annealing, a local minimum is found by minimizing the GRS loss function in LAMMPS (the effective potential on the y-axis).}
    \label{fig:min_method}
\end{figure}


More advanced global optimization algorithms could help guarantee a single structure best reproduces an arbitrary target descriptor distribution. However, pursuing these may not be worth the extra computational expense these impart. 
The key problem will often remains that many target distributions cannot be represented well by a single atomic structure. This is especially true if one needs structures near or below 100 atoms for use in electronic structure theory; these may be significantly to small to accurately reproduce complex target distributions of descriptors. 
Instead of a single representative structure, a set of representative structures may be produced to more accurately and effectively span a target distribution.
The ability to do this for multiple initial structures is embarrassingly parallelizable and makes this approach amenable to global optimization methods that rely on generations of candidate structures such as genetic algorithms and basin-hopping. 


%This includes molecular dynamics, iterative optimization algorithms, and Monte Carlo, which are all useful for minimizing structures on the GRS loss surface. 
%Note that poor guesses of initial structure will result in these optimization algorithms incorrectly assigning local minima as global minima. This shortcoming can be mitigated by combining the local optimization algorithms in LAMMPS with global optimization algorithms and parallel sampling methods. 
%While careful selection of starting structures can aid in finding a global minimum to the GRS loss function, methods that are better suited for finding global minima are sometimes needed. 




%This figure shows atomic structures sampled in searches as well as states sampled by CG once annealing is finished to find the local minimum.



%\subsubsection{}

\subsection{Stochastic optimization}
%Different sampling methods may be used to optimize the structures and minimize GRS loss function. 
%So far, the method used is specified before minimizing the GRS loss function, but in the future this may be determined on-the-fly based on the target distribution of ACE descriptors. 
Similar to how the candidate structure types are specified based on the target distribution of ACE descriptors, the sampling and optimization methods are as well. In general, GRS and GRSS are obtained by combining algorithms that can find global minima with algorithms for to find local minima. In general, this must be done by optimizing both the atomic positions and chemical occupations. Depending on the target, favoring either spatial or chemical degrees of freedom or one optimization algorithm over the other may be advantageous. 
For example, targets corresponding atomic structures that lie on (or close to) a fixed parent lattice are sampled with chemical occupation flips or chemical occupation swaps. It is more efficient to find representations of such targets with only SA or genetic algorithms (GA) rather than including a local optimization method like CG.
Thus, GRS targeting varied local chemistries is performed as it is for fixed-lattices in SQS through chemical occupation flips or swaps.\cite{van2013efficient} If atomic positions cannot be fixed based on the target distribution, methods to find local minima are wrapped by the the chemical sampling (the SA or GA optimizer).

%In cases where the target distribution corresponds to irregular or disordered atomic sites, the positional degrees of freedom may be sampled more regularly. While sampling atomic positions can be done in SA, GA, and or in stochastic methods, it is often inefficient. 
%Conversely, iterative optimization algorithms such as conjugate gradient are better suited. For targets resembling amorphous, liquid, and other disordered off-lattice systems, conjugate gradient is employed through LAMMPS to optimize atomic positions. 
%These iterative optimizers are used in conjunction with the stochastic methods like SA and GA. The stochastic method samples the chemical degrees of freedom while the iterative optimizer pushes atomic coordinates such that the structures reach local minima on the GRS loss surface.

For targets spanning both chemical and spatial degrees of freedom a mix of chemical and spatial sampling is performed. The amount of spatial vs chemical sampling is controlled, in part, through the types of candidate structures proposed, but also through randomly chosen chemical versus spatial sampling. 
The random sampling of chemical versus spatial degrees of freedom is specified through: (1) the probability of moving and/or optimizing atomic positions through iterative optimizers and (2) the probability for sampling new chemical occupations through chemical occupation flips, swaps, or a different candidate structure. 
\begin{equation}
    P_{All}= P_{chem.} + P_{spatial} = 1.0
    \label{eq:probabilities}
\end{equation}
The probability of sampling chemical vs spatial degrees off freedom is defined simply with Eq. \eqref{eq:probabilities}. These probabilities are specified based on the target. In some cases, one of the sampling degrees of freedom may be set to zero. For example, the GRS method may be used to generate structures on a fixed parent lattice. In those cases $P_{spatial}=0$.

For the stochastic optimization methods for minimizing loss-functions, GA and SA are used.\cite{forrest1993genetic} 
The mutations in the GA and the Monte Carlo steps in the SA method are comprised of (1) random spatial steps of atomic coordinates for one atomic site (2) chemical occupation flips for an atomic site, (3) chemical occupation swaps for two atomic sites.
These moves may be chosen based on the target distribution and constrained.
For example, if the target is an alloy with a fixed composition of $A_{0.5}B_{0.5}$, the occupation flips/swaps may be constrained to maintain this global chemical composition and the random atomic position movements turned off to preserve the lattice structure.

For the GA, two different crossover functions may be used. One crossover function combines a fraction of one structures atomic coordinates and chemical occupations with the coordinates and chemical occupations of a second structure. 
This is accomplished by collecting a random slice of atoms from two parent structures and combining them in one of the parent cells. If this results in atomic overlap, one of the overlapping atoms is removed. The second crossover function used takes the atomic coordinates from only one parent, but allows for mixing of the chemical occupations.
From a given generation of atomic structures, candidates were selected using a tournament selection method. The GRS loss function is used directly in the tournament selection method to evaluate the fitness of the candidates.

For the SA optimizer, the allowed steps are specified based on the target distribution (e.g. chemical vs spatial). Beyond these steps that were defined earlier along with the GA "mutations", the simulated annealing method is characterized by the acceptance criteria. In this case, the acceptance criteria is defined in terms of differences in the GRS loss function from one Monte Carlo step and the previous step.
\begin{equation}
    \mathrm{argmin} \bigg(1,  \;\; exp\big(-\beta [Q_{GRS}^1 - Q_{GRS}^0 ]\big) \bigg)
    \label{eq:sa_criteria}
\end{equation}
In Eq. \eqref{eq:sa_criteria}, the acceptance criteria for SA is given in terms of the GRS loss function at different Monte Carlo steps and a thermodynamic beta, $\beta$ that artificially introduces temperature. 
The beta is initialized such that it corresponds to an large initial temperature. After a sufficient number of steps, it is decreased. This procedure is similar to what is done for SQS.

Either the SA or the GA is used within for global optimization when necessary. 
A comparison of the global optimization methods is given in the results for a key demonstration of GRS.
For the majority of the applications the GA is applied, or at least an single generation of atomic structures from the GA is used for parallel sampling.
In some cases, accurate representative structures may still be obtained using only the CG method in LAMMPS, provided that appropriate candidate structures are proposed.
%A target distribution resembling a fairly well defined crystal lattice will be sampled more heavily in chemical degrees of freedom and the initial structure will resemble the same parent lattice, as determined by symmetry detection libraries.\cite{spglib}  

%Target distributions that lack long-range translational symmetry will have spatial degrees of freedom sampled heavily. The starting structures for a disordered system such as this will be a hermite-normal-form supercell of a relevant parent lattice symmetry, but with randomized atomic positions, or as with the original SQS method, a specified supercell. More information about the random structure generation procedures can be found in the supporting information.

%For systems lacking long-range translational symmetry with many chemical degrees of freedom, it has been found that performing an grand canonical loop to approach ideal or specified stoichiometry, then fixing the composition and doing only canonical swaps greatly increases the rate of convergence of a GRS structure.

%\subsection{Radial distribution functions}

\subsection{Initial candidate structures}
Given the broad range of target distributions accessible with GRS, it is important to have reasonable initial guesses for structures. If not, reasonable minima may not be found. The same is true for SQS methods and this does not diminish the utility of SQS.
In SQS, the residual of the SQS loss function (the minimal value of the SQS loss function) is related to cell size and the target distribution and initial candidate structures should are chosen with some consideration of the target .\cite{van2009multicomponent,van2013efficient,aangqvist2019icet,zunger1990special} 
For example, when the target in SQS is a random alloy, a randomly occupied supercell is often used as an initial candidate structure. More accurate representations of the random alloy target may be obtained with larger supercells.

Currently candidate structures in GRS are also proposed according to the target distribution of ACE descriptors. Target distributions of ACE descriptors corresponding to fixed-lattice systems are assigned with random atomic positions close to those from the parent lattice. 
The parent lattice may be identified through an appropriate ACE descriptor set or, if a single atomic structure is set as the target, by atomic structure symmetry libraries.\cite{togo2024spglib}
Liquid and amorphous systems are assigned randomly occupied supercells with variable density close to those sampled by the target. 
Chemical occupations are typically assigned randomly and according to restrictions based on global composition.
There is flexibility in the candidate structures proposed in both spatial and chemical degrees of freedom.
The sizes, shapes, and chemistries of supercells may be specified. For example, one may restrict candidates to be $2\times 2 \times 2$ BCC supercells.

If more flexibility in spatial degrees of freedom is required, supercells of arbitrary parent lattices may be generated using Hermite normal form transformations, similar to the first step in Ref.~[\citenum{morgan2017generating}].
More thorough spanning of chemical occupations may be accessed by using fixed-lattice candidates generated with existing algorithms, or similar methods to span unique chemical labelings of supercells.\cite{morgan2017generating,aangqvist2019icet}  
The classes of initial candidate structures used presently for GRS are obviously not exhaustive of all possible atomic configurations. However, as is demonstrated in our results, the current variability in candidate structures is sufficient for starting the GRS optimizations with diverse solid-state targets.
Candidates relevant for molecular and organic systems could easily be introduced using analogous arguments for domain expertise and symmetry. However, the initial candidate structure types already presented may be useful for some coarse-grained molecular systems.

\subsection{ACE descriptor selection}
The ACE descriptor sets in theory are complete, but in practice the body order of ACE descriptors needs to be truncated much like the fixed-lattice cluster functions. Unlike the fixed-lattice cluster functions, the radial and angular basis functions used to construct ACE descriptors need to be truncated per body order. Additionally, hyper-parameters for the radial basis need to be specified; by default with the LAMMPS interface, this requires specifying hyper-parameters for the radial basis used in Ref.~\citenum{drautz_atomic_2019}. 
The radial function cutoffs are specified based on tabulated Van der Waals radii.\cite{larsen2017atomic} For most relevant condensed matter systems considered within, this corresponded to 4-7 neighbor shells.
The scaled distance decay parameters, $\lambda$ in Ref.~\citenum{drautz_atomic_2019}, were specified to be 5\% of the radial cutoff. Many other values of radial cutoffs and radial decay parameters were tested for single and multi-element target systems. The 5 \% fraction was chosen because it showed improved information content compared to other hyper-parameter choices with lower global feature reconstruction errors.\cite{goscinski2023scikit} It is noted that the parameters corresponding to an optimized ACE interatomic potential may differ.\cite{bochkarev_efficient_2022}
To truncate the body order of the ACE descriptor sets, complete sets of ACE descriptors up to 5-body (rank 4) are enumerated.\cite{goff2024permutation} The maximum radial function indices per descriptor rank are: $n_{max}=8,2,2,1$ and angular $l_{max}=0,2,2,1$.
For the 4-element Fe-Cr-Si-V system, the same set is used,  but it is truncated at 4-body.

==> methods_maw.tex <==
\section{Methodology}

A structure represented by atomic descriptors can be compared to any other structure and a quantitative mismatch given in terms of the loss function in Eq. \ref{eq:inter_structure}.
Similarly, a set of structures can be represented with a descriptor distribution, and the mismatch with another descriptor distribution quantified, the loss function in Eq. \eqref{eq:intra_structure}. 
Structures that best reproduce a reference distribution are the GRS, and are defined as those that minimize these loss functions. More generally, the summation of Eq. \ref{eq:inter_structure} and Eq. \ref{eq:intra_structure}, with associated weighting terms give the target optimization for GRS, Eq. \ref{eq:grs_set_def}. Generalized representative structures are defined as those obeying
\begin{equation}
    \min_{(R_{s_1}\sigma_{s_1}),(R_{s_2}\sigma_{s_2}), \cdots (R_{s_{N_s}}\sigma_{s_{N_s}})}\big[w_1 Q_{GRS} + w_2 Q_{GRS}^{intra} \big].
    \label{eq:grs_set_def}
\end{equation}
In practice the atomic positions (${R_s}$) and chemical identities (${\sigma_s}$) are not easily intuited, and require optimization until any local or global minima of Eq. \ref{eq:grs_set_def} are to be found. 
The following subsections address each of the key practical concerns that enable GRS generation, followed by practical application of the method.
A pictorial representation of the overall challenge is given in Figure \ref{fig:min_method} where a desired descriptor distribution (purple star) lives at a minima of some effective potential that only depends on the values of the candidate structural and chemical descriptors. 
Proposing an initial candidate structure (grey circle), global optimization steps (blue circles) and local optimization routines (orange circles) that minimize Eq. \ref{eq:grs_set_def} in a computational efficient means are discussed within.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{GRS_min.001.jpeg}
    \caption{Illustration that highlights the optimization of the GRS loss function for a single atomic structure. An initial structure is annealed on the loss surface are by varying atomic positions and chemical occupations (encoded in the fingerprints on the x-axis). After annealing, a local minimum is found by minimizing the GRS loss function in LAMMPS (the effective potential on the y-axis).}
    \label{fig:min_method}
\end{figure}

\subsection{Effective potential}
As stated previously, the GRS distinguishes itself from traditional structure optimization methods in that an energy model is not needed \textit{a priori}.
Instead atoms are evolved by utilizing the loss function plus a constraint to avoid close atom contacts,
\begin{equation}
    \begin{split}
    &V^{eff}({\{ \boldsymbol{R}}\}_S,\{\boldsymbol{\sigma}\}_S )=V_{core}({\boldsymbol{R}},\boldsymbol{\sigma})  + w_{1}Q_{GRS}({\boldsymbol{R}_s},\boldsymbol{\sigma}_s ) \\
    & + w_{2}Q_{GRS}^{intra}({\{ \boldsymbol{R}}\}_S,\{\boldsymbol{\sigma}\}_S ).
    \end{split}
    \label{eq:multi_eff}
\end{equation}
Equation \ref{eq:multi_eff} accounts for the interactions among atoms in a single structure, $({\boldsymbol{R}},\boldsymbol{\sigma}$), as well as across multiple structures $\{\boldsymbol{R},\boldsymbol{\sigma}\}$ that contribute to their respective loss functions $Q_{GRS}$.
Note the dependent variables are used to calculate the ACE descriptors which are smooth and continuous with respect to ${\boldsymbol{R}}$ and $\boldsymbol{\sigma}$, we utilize the efficient LAMMPS implementation of this basis set.\cite{thompson2022lammps,lysogorskiy_performant_2021}

Methods for sampling chemical degrees of freedom in atomic systems are typically well-established stochastic approaches, but this is not efficient for the continuous domain of atomic positions that need to be sampled in GRS methods. 
The key advance enabling optimization of GRS loss functions with dynamic atomic positions is the new ACE capabilities in the machine-learned interatomic potential (ML-IAP) interface in LAMMPS.
This allows a user to define the interaction model in Python without the need to make compiled language (C++) changes to the LAMMPS code base.
ACE descriptors are passed to the external interaction model, where LAMMPS receives per-atom energies and forces needed to perform molecular dynamics, minimization, or any other operations that LAMMPS supports.
Local minima may easily be found on \eqref{eq:multi_eff} by optimizing atomic positions according to conjugate gradient (CG), steepest descent algorithms, and other optimization algorithms used for molecular dynamics.
A key problem will often remains that many target distributions cannot be represented well by a single atomic structure. This is especially true if one needs structures near or below 100 atoms for use in electronic structure theory; these may be significantly to small to accurately reproduce complex target distributions of descriptors. 
A set of representative structures may be found by starting with one GRS, adding new candidate structures to the set $S$, and evolving atomic positions such that they minimize the effective potential Eq. \eqref{eq:multi_eff}.

\subsection{Stochastic sampling}
In general, sets of GRS are obtained by combining algorithms that can find global minima with those for local minima.
Depending on the target, favoring either spatial or chemical degrees of freedom or one optimization algorithm over the other may be advantageous. 
For example, targets corresponding atomic structures that lie on (or close to) a fixed parent lattice are sampled with chemical occupation flips or chemical occupation swaps. It is more efficient to find representations of such targets with only SA or genetic algorithms (GA)\cite{forrest1993genetic} rather than including a local optimization method like CG.
Thus, GRS targeting varied local chemistries is performed as it is for fixed-lattices in SQS through chemical occupation flips or swaps.\cite{van2013efficient} 
If atomic positions cannot be fixed based on the target distribution, methods to find local minima are wrapped by the the chemical sampling.
The amount of spatial vs chemical sampling is controlled, in part, through the types of candidate structures proposed, but also through randomly chosen chemical versus spatial sampling. 
The random sampling of chemical versus spatial degrees of freedom is specified through: (1) the probability of moving and/or optimizing atomic positions through iterative optimizers and (2) the probability for sampling new chemical occupations through chemical occupation flips, swaps, or a different candidate structure. 
Where the parent lattice is known, or a single chemistry is desired, one can nullify one of these probabilities.

For the GA, two different crossover functions may be used. One crossover function combines a fraction of one structures atomic coordinates and chemical occupations with the coordinates and chemical occupations of a second structure. 
This is accomplished by collecting a random slice of atoms from two parent structures and combining them in one of the parent cells. If this results in atomic overlap, one of the overlapping atoms is removed. The second crossover function used takes the atomic coordinates from only one parent, but allows for mixing of the chemical occupations.
From a given generation of atomic structures, candidates were selected using a tournament selection method. The GRS loss function is used directly in the tournament selection method to evaluate the fitness of the candidates.

For the SA optimizer, the allowed steps are specified based on the target distribution (e.g. chemical vs spatial). Beyond these steps that were defined earlier along with the GA "mutations", the simulated annealing method is characterized by the acceptance criteria. In this case, the acceptance criteria is defined in terms of differences in the GRS loss function from one Monte Carlo step and the previous step as
\begin{equation}
    \mathrm{argmin} \bigg(1,  \;\; exp\big(-\beta [Q_{GRS}^1 - Q_{GRS}^0 ]\big) \bigg).
    \label{eq:sa_criteria}
\end{equation}
In Eq. \eqref{eq:sa_criteria}, the acceptance criteria for SA is given in terms of the GRS loss function at different Monte Carlo steps and a thermodynamic beta, $\beta=1/k_b T$ that artificially introduces temperature. 
The beta is initialized such that it corresponds to an large initial temperature. After a sufficient number of steps, it is decreased. This procedure is similar to what is done for SQS.

Either the SA or the GA is used within for global optimization when necessary. 
For the majority of the applications the GA is applied at least a single generation of atomic structures from the GA is used for parallel sampling.
In some cases, accurate representative structures may still be obtained using only the CG method in LAMMPS, provided that appropriate candidate structures are proposed.

\subsection{Initial conditions}
Given the broad range of target distributions accessible with GRS, it is important to have reasonable initial guesses for structures. If not, reasonable minima may not be found. 
For comparison, the residual of the SQS loss function (the minimal value of the SQS loss function) is related to cell size and the target distribution and initial candidate structures should are chosen with some consideration of the target .\cite{van2009multicomponent,van2013efficient,aangqvist2019icet,zunger1990special} 
When the target in SQS is a random alloy, a randomly occupied supercell is often used as an initial candidate structure. More accurate representations of the random alloy target may be obtained with larger supercells.

Currently, candidate structures in GRS are also proposed according to the target distribution of ACE descriptors. 
Target distributions of ACE descriptors corresponding to fixed-lattice systems are assigned with random atomic positions close to those from the parent lattice. 
The parent lattice may be identified through an appropriate ACE descriptor set or, if a single atomic structure is set as the target, by atomic structure symmetry libraries.\cite{togo2024spglib}
Liquid and amorphous systems are assigned randomly occupied supercells with variable density close to those sampled by the target.
Chemical occupations are assigned randomly and according to restrictions based on global composition.
If more flexibility in spatial degrees of freedom is required, supercells of arbitrary parent lattices may be generated using Hermite normal form transformations, similar to the first step in Ref.~[\citenum{morgan2017generating}].
More thorough spanning of chemical occupations may be accessed by using fixed-lattice candidates generated with existing algorithms, or similar methods to span unique chemical labelings of supercells.\cite{morgan2017generating,aangqvist2019icet}  
The classes of initial candidate structures used presently for GRS are obviously not exhaustive of all possible atomic configurations. However, as is demonstrated in our results, the current variability in candidate structures is sufficient for starting the GRS optimizations with diverse solid-state targets.
Candidates relevant for molecular and organic systems could easily be introduced using analogous arguments for domain expertise and symmetry. However, the initial candidate structure types already presented may be useful for some coarse-grained molecular systems.

Lastly, the initial conditions of the ACE basis set that underpin all of these sampling methods needs to be defined. 
The ACE descriptor sets in theory are complete, but in practice the body order needs to be truncated much like the fixed-lattice cluster functions. 
Unlike the fixed-lattice cluster functions, the radial and angular basis functions used to construct ACE descriptors need to be truncated per body order. 
Additionally, hyper-parameters for the radial basis need to be specified; by default with the LAMMPS interface, this requires specifying hyper-parameters for the radial basis used in Ref.~\citenum{drautz_atomic_2019}. 
The radial function cutoffs are specified based on tabulated van der Waals radii.\cite{larsen2017atomic} 
For most relevant condensed matter systems considered within, this corresponded to 4-7 neighbor shells.
The scaled distance decay parameters, $\lambda$ in Ref.~\citenum{drautz_atomic_2019}, were specified to be 5\% of the radial cutoff. 
Many other values of radial cutoffs and radial decay parameters were tested for single and multi-element target systems. 
The 5 \% fraction was chosen because it showed improved information content compared to other hyper-parameter choices with lower global feature reconstruction errors.\cite{goscinski2023scikit} 
It is noted that the parameters corresponding to an optimized ACE interatomic potential may differ.\cite{bochkarev_efficient_2022}
To truncate the body order of the ACE descriptor sets, complete sets of ACE descriptors up to 5-body (rank 4) are enumerated.\cite{goff2024permutation} 
The maximum radial function indices per descriptor rank are: $n_{max}=8,2,2,1$ and angular $l_{max}=0,2,2,1$.
For the 4-element Fe-Cr-Si-V system, the same set is used, but it is truncated at 4-body.

